Adversarial Perturbations of Opinion Dynamics in Networks

We study the connections between network structure, opinion dynamics, and an adversary's power to artificially induce disagreements. We approach these questions by extending models of opinion formation in the social sciences to represent scenarios, familiar from recent events, in which external actors seek to destabilize communities through sophisticated information warfare tactics via fake news and bots. In many instances, the intrinsic goals of these efforts are not necessarily to shift the overall sentiment of the network, but rather to induce discord. These perturbations diffuse via opinion dynamics on the underlying network, through mechanisms that have been analyzed and abstracted through work in computer science and the social sciences. We investigate the properties of such attacks, considering optimal strategies both for the adversary seeking to create disagreement and for the entities tasked with defending the network from attack. We show that for different formulations of these types of objectives, different regimes of the spectral structure of the network will limit the adversary's capacity to sow discord; this enables us to qualitatively describe which networks are most vulnerable against these perturbations. We then consider the algorithmic task of a network defender to mitigate these sorts of adversarial attacks by insulating nodes heterogeneously; we show that, by considering the geometry of this problem, this optimization task can be efficiently solved via convex programming. Finally, we generalize these results to allow for two network structures, where the opinion dynamics process and the measurement of disagreement become uncoupled, and determine how the adversary's power changes; for instance, this may arise when opinion dynamics are controlled an online community via social media, while disagreement is measured along "real-world" connections.

==> intro.tex <==
% !TEX root = main.tex
\section{Introduction}


People's opinions are shaped by their interactions with others.
The resulting process of {\em opinion dynamics} --- the interplay
between opinion formation and the network structure of these
interactions --- has been of great interest in the political science,
sociology, economics, and computer science communities among others.

A range of mathematical models have been proposed for opinion
dynamics in social networks, representing people as nodes in the network.
In typical models, each node in a weighted graph $G=(V,E)$ holds
a real-valued opinion that updates in response to
the values in their network neighborhood. 
In perhaps the most natural model, the
repeated-averaging model of DeGroot, each node repeatedly takes a weighted
average of its own opinion with those of its neighbors; using rich connections between stochastic matrices and Markov chains, it
is possible to show that these dynamics lead to all individuals
sharing a \emph{consensus} opinion in the limit
\cite{degroot1974reaching}. Much work in the economics and social science
literature has studied fundamental questions in this basic model
\cite{golub2010naive}.

A typical feature of real-world networks, however, is that even
approximate consensus is rarely, if ever, achieved. For that reason,
richer models like the Friedkin-Johnsen variation of the
standard DeGroot model \cite{friedkin1990social} or the
bounded-confidence Hegselmann-Krause model
\cite{hegselmann2002opinion} have been proposed to give plausible
explanations for how these long-term disagreements can persist while
maintaining the strong intuition that one will account for and adjust
to the opinions and expressed behaviors of those near them. In this
work, we will take the Friedkin-Johnsen model as a primitive; these
dynamics closely follow the basic DeGroot model, but allow each node
to hold their own immutable internal opinion which always gets
incorporated during the repeated averaging.\\

\textbf{Discord and Adversarial Perturbations.}
These types of mathematical models have been used extensively to study 
both the phenomena associated with consensus and polarization,
as well as the role of interventions designed to shift opinions, 
in which targeting a few individual opinions can shift many others
via the network dynamics.
While the questions have been quite diverse, they share
a crucial underlying assumption, which is that the entities
intervening in the process have a preferred opinion that they
are seeking to promote.

In the real-world settings that motivate these models, however,
a number of important developments have been commanding increasing
attention in the past few years.
One of these is the rising concern about situations in which outside
entities intervene not to promote a specific opinion, but 
instead to induce a {\em lack} of consensus, 
with the explicit intention of
sowing discord. For instance, the U.S. Department of Justice Special
Counsel's Office argues in their 2017 indictment of the Russian
Internet Research Agency (IRA) that the IRA used social media and
targeted advertising with ``a strategic goal to sow discord in the
U.S. political system, including the 2016 U.S. presidential election''
\cite{iraindictment}. This behavior has been seen in multiple countries,
and is not limited to any one actor. 
For example, the doctrine of offensive information warfare by the U.S. 
intelligence community includes provisions for the instigation
of discord between opposing parties \cite{nrc-covert-action}.
More recently, Twitter
disclosed in 2019 that external bots made a coordinated effort to ``sow
political discord in Hong Kong'' with the aim of making protesters
less effective at organizing during the Hong Kong independence
movement \cite{twitter_2019}. It is to be expected that as social
media becomes more and more prevalent, these sorts of external
influences and behaviors will become more frequent.

In such instances, the apparent aim of these attacks is not directly
to promote a specific policy agenda, but rather simply to induce
disagreement; correspondingly, these external actors strive for more
abstract objectives and therefore exhibit more complicated behavior.
For example, analysis of Twitter data in the past few years has
revealed how bots sponsored in some cases by state actors
managed to play both sides of some existing
issue to exploit divisions along racial lines, pro- and anti-vaccine
groups, NFL kneeling, and gun reform, among other matters
\cite{senatereport, broniatowski2018weaponized,diresta2019tactics}.

For these types of scenarios, in which an adversary is seeking
to promote disagreement, we need to look beyond existing 
mathematical formulations of opinion maximization and influence in networks.
We show how to define a new set of questions in the
underlying models of opinion dynamics based on an adversary whose
objective function is some measure of node-to-node disagreement.
In this paper, we formalize such questions; 
roughly speaking, we will start from instances of the 
Friedkin-Johnsen model in which all nodes' internal opinions are at equilibrium, e.g., they are all
equal to $0$, and then we will allow an adversary to perturb
these internal opinion subject to some radius constraint modeling resource constraint of the attacker.
These seeded
internal opinions then diffuse across the 
network to reach an equilibrium under the Friedkin-Johnsen dynamics, 
at which point some measure of disagreement among adjacent nodes is
measured.
Our main goal is to characterize the
interplay between graph structure and the adversary's power: which
networks are most susceptible to or resilient to these kinds of 
perturbations; how can the adversary most efficiently spend 
a bounded amount of resource in order to produce the maximum disagreement;
and how can we most effectively defend a network against such attacks?
We will find that these types of questions bring into play
new network properties that have not typically arisen in 
the analysis of traditional questions around consensus, polarization,
and opinion maximization.

\subsection{Our Results}

\textbf{Spectral Properties of Discord.} In this work
an adversary seeking to maximize 
some measure of {\em discord} among the nodes of a network
would like to perturb the internal opinions of the nodes by
a bounded amount in order to produce as much discord as possible
under the resulting opinion dynamics.

We first show that many such
objectives for such an actor can be naturally posed as the
maximization of an associated quadratic form of the underlying graph
Laplacian. The simple, but crucial observation is that {this
directly connects the adversary's power in attaining their objective
with the eigenvalues of some function of the underlying graph}. The
graph Laplacian is an extremely well-studied object, whose spectral
properties are known to be good approximations of combinatorial
features of the underlying network; this connection will allow us to
qualitatively understand what structural properties of the graph
matter in these different settings.

For different discord objectives, we find that
different regimes of the spectral structure of the underlying networks
characterize the ability of this adversary to succeed in their aim.
In perhaps the most natural case, we define the disagreement 
on an edge of the network to be the squared difference of the opinions
at the edge's endpoints; and we define the disagreement of the network
to be the sum of the disagreements on all its edges.
The challenge for an adversary in maximizing disagreement is that
the same network is being used both by the opinion dynamics to
average away the disagreement, and by the objective function to measure
the disagreement.
We can study this effect in terms of a key one-dimensional parameter
$t$ inherent in the Friedkin-Johnsen opinion dynamics model,
controlling the relative weight of a node's internal opinion and
neighboring opinions in determining how it updates its opinion
in the next time period.
We find, strikingly, that as $t$ ranges from $0$ to $\infty$,
the optimal strategy for the adversary is determined by a sequence
of vectors that ranges over precisely the set of eigenvectors of
the graph Laplacian.
This means that for an adversary seeking to induce maximum disagreement,
the \emph{entire} eigenstructure of the network is relevant.

This dependence on the entire eigenstructure forms a strong contrast
with standard graph objective functions that have a spectral interpretation,
where we typically find a dependence only on the extreme eigenvectors.
Here, by contrast, {\em each} eigenvector controls the optimal choice
for the adversary at some setting of the opinion dynamics.

We also consider additional discord objectives, finding that
the contrast extends here too, with the adversary's optimal behavior
for these other objectives dependent on extreme eigenvectors.
In particular, when the adversary's objective is to maximize
the polarization-disagreement index of Musco, Musco, and Tsourakakis
\cite{musco2018minimizing}, the ability of the adversary is directly
controlled by the second smallest eigenvalue of the graph Laplacian.
Somewhat surprisingly, an infinite-time horizon form of the maximum
disagreement objective is also completely determined by the second
smallest eigenvalue, despite not holding for the one-period time
horizon mentioned above. Through these well-studied connections
between the spectral and combinatorial structures of graphs, we can
then qualitatively describe which networks, under the Friedkin-Johnsen
dynamics, are robust to these sorts of adversarial perturbations.\\

\textbf{Network Defense.} In Section \ref{section:defense}, we
generalize the basic model and consider the converse problem of
\emph{minimizing} the ability of such an adversary to promote
their objective. Following the general principle that the network
topology ought be somewhat difficult to meaningfully change, we allow
a network defender to \emph{insulate} the individuals in the network
heterogeneously. Intuitively, this corresponds to making these
individuals more difficult for an adversary to influence via their
internal opinion. This might be achieved, for instance, through
technological literacy initiatives to make it more difficult for
certain individuals to be susceptible to the normal modes by which an
external actor may seed internal opinions, like bots or fake news.

Formally, we will consider a two-player min-max game, where a network
defender can first heterogeneously \emph{weigh} different individuals
in the network (subject to some explicit normalization); the
interpretation is that the defender can make some individuals less
malleable to seeding. The adversary then solves their objective
function as before, but subject to these new weights. The constraints
on the defender's choice will include the option to keep the
individuals' weights the same as above, so that this optimization
problem for the defender is upper-bounded by the previous analyses. On
the algorithmic side, our main technical contribution in this section
is to show that while the adversary's inner maximization problem no longer has the well-known analytic connection to eigenvalues, for many choices of the adversary's objective and
weight normalization, the network defender's problem can be globally
solved using convex programming. We show this by analyzing the geometry of the defender and adversary's optimization problems. In particular, this implies
the network defender's problem can be solved efficiently.\\

\textbf{Mixed-Graph Objectives.} 
As noted above, the underlying network is playing two distinct
roles in our basic model of disagreement: 
it serves to average opinions of neighboring nodes, and it also 
serves to measure the disagreement between neighbors in the
resulting equilibrium of the opinion dynamics.
But if we look at current discussions of the ways in which
online interaction may be exacerbating conflict among different
opinions, a crucial theme is the way in which the online content
that shapes our opinions is being transmitted across networks that
may be quite different from the social networks linking us to the
people with whom we interact on a daily basis.

These considerations suggest that we return to the adversary's
disagreement maximization
problem, but when the network where disagreement is measured can be different
from the network where the Friedkin-Johnsen opinion dynamics take
place. The individuals and communities one interacts with on social
media can be quite global in nature, as well as relatively anonymous
and self-selecting; in contrast, one's real-world interactions are far
more dictated by other factors like geography and occupation. It is
thus quite natural to think of opinion formation as occurring somewhat
orthogonally to these real-world interactions. To sow discord, an
adversary might hope to induce disagreement measured via these
real-world connections, but must do so filtered through the opinion
dynamics in the online world. Intuitively, if
the opinion graph which does the smoothing of internal opinions and
the disagreement graph look very different, an adversary will be much
more powerful than what is possible in the basic model 
when these graphs must be the same.

To understand this setup, we generalize the adversary's problem with
\emph{mixed-graph} objective functions in the natural way by
considering two distinct graphs at once. One might expect that the
adversary is most limited when the opinion graph and disagreement
graphs are the same, as then the opinion dynamics smooth out the
seeded opinions along the exact same network where disagreements will
be measured. Somewhat surprisingly, we show that it is not always the
case, even subject to some natural degree normalization; there are
explicit, simple disagreement graphs where a different opinion
formation graph provably lowers the adversary's ability to induce
disagreement by a non-negligible amount. However, we also give a
general lower bound that suggests that these examples are somewhat
pathological in that, typically, having different graphs will help the
adversary in this aim compared to the single-graph setting. For other
disagreement graphs, it will in fact turn out that they are optimal
for themselves.

On the one hand, if the measurement and disagreement graphs are highly
similar, edge-by-edge, then the adversary's basic optimization problem
has not really changed from the single-graph setting. This is indeed
the case, via an easy continuity argument, but \emph{not necessary}.
To that end, we show that if the two graphs are good spectral
approximations for each other, then the objective of the adversary is
essentially unchanged. It is well-known using celebrated results of
Batson, Spielman, and Srivastava the every graph, no matter how dense,
has a spectral approximation corresponding to much sparser graph
\cite{batson2012twice}. In particular, this implies that it is not
necessary at all for the two graphs to be \emph{physically} quite
similar, only \emph{spectrally} quite similar.

In the converse direction, it is still quite intuitive that the more
dissimilar the two graphs are, the more an adversary will be able to
induce disagreement. We show that spectral dissimilarity,
appropriately defined, is sufficient for this purpose. Perhaps more
interestingly, by specializing to combinatorial structure, it will
follow that if the two graphs are misaligned in the sense that their
cut structure differs by a large amount along any subset of nodes,
then necessarily the adversary is far more capable of inducing
disagreement than in the single-graph setting. This provides some
theoretical justification for why external actors have been able to
effectively sow discord; this can happen when opinion formation and
disagreement become uncoupled, as is possible with social media platforms.

\subsection{Related Work}

\jgedit{To our knowledge, the focus on interventions to increase discord
in the Friedkin-Johnsen model is new.} In its emphasis on interventions in such models more generally, 
our work has connections to that of
Gionis, et al \cite{gionis2013opinion}. In their work, the authors establish
the $\mathsf{NP}$-hardness of a natural opinion \emph{maximization}
problem work in the Friedkin-Johnsen dynamics. They also derive a
random walk interpretation of these dynamics to establish
submodularity of their problem, enabling a polynomial-time
$(1-1/e)$-approximation algorithm using the natural greedy algorithm.
We focus on different optimization tasks motivated by recent
events aimed at sowing discord in opinion dynamics, 
and moreover, we do not focus on the computational hardness of
such tasks. Indeed, in our setting, the optimization problems will be
computationally tractable. Instead, our emphasis will be on the
relationship between the graph and the adversary's power in achieving
their aims.

Subsequent work by Musco, Musco, and Tsourakakis
\cite{musco2018minimizing} considered a problem, given either a
fixed graph topology or fixed initial opinions, of determining the
optimal choice of the other to minimize their
polarization-disagreement index metric. Their main results shows that
both of these problems can be efficiently solved via convex
optimization. Our approach deviates from theirs in multiple ways: for
one, motivated by these recent events, we are interested in a
\emph{worst-case}, adversarial analysis, not in finding best-case
settings. Moreover, our general philosophy is that the graph topology
for the dynamics is typically quite immutable; the problems we
consider will treat the underlying graphs as fixed. We will also be
principally concerned with analytically characterizing an adversary's
power in these settings in relation to the underlying graph. In a
different direction, prior work by Bindel, Kleinberg, and Oren
interprets the Friedkin-Johnsen dynamics as the Nash equilibrium of a
natural quadratic cost function \cite{bindel2015bad}; they then
characterize the price of anarchy of this equilibrium, namely the
ratio between the cost at equilibrium with that of the global
optimizer. By using spectral techniques, they establish an upper bound
of $9/8$ on this ratio, thereby showing that the equilibrium solution
is a good minimizer of the global cost function.

 \jgedit{Closest to the motivation for our work is an independent paper by Chen and Racz \cite{chen2020network} who consider the power of an adversary seeking to induce discord, but subject to a sparsity constraint. We explain the connections between our approach and theirs in Section \ref{sec:racz}, and demonstrate how combining our spectral approach with their analysis can sharpen some of the results in their setting.}
 

Our current work has thematic elements of all these  papers;
motivated by current events, we consider optimization
tasks in these dynamics. 
As mentioned above, we will largely view the underlying
graph topology as fixed,  and we will consider instead the ability of
an adversary to induce discord by supplying internal opinions
on some issue that previously was at consensus. We will be primarily
concerned with the interplay between graph structure and the
adversary's ability to do so. The opinion dynamics serve to
equilibrate any seeded opinions by an external actor, thus dampening
the effect of the adversary; however, the connections in the graph can
also heighten the resulting disagreement. We also study these
competing effects using primarily spectral techniques and convex
optimization. The network defense problem and mixed-graph objectives
we consider are, to the best of our knowledge, novel to this
literature. These models allow for opinion dynamics and disagreement
to be slightly orthogonal processes and cannot be completely
characterized using the spectral theory of a single graph Laplacian.
We hope that these kinds of generalizations may prove an interesting
direction for future work.

